An Adaptive Channel Reservation MAC Protocol Based on Forwarding Traffic of Key Nodes

Ad Hoc networks with multi-hop topology are widely used in military and civilian applications. One challenge for Ad Hoc networks is to design efficient Media Access Control (MAC) protocols to ensure the quality of service (QoS). In Ad Hoc networks, there is a kind of node called key node, which undertakes more forwarding traffic than other surrounding nodes. The number of neighbor nodes around key nodes is often large, and the surrounding channel environment and interference are often more complex. Thus, the key nodes can hardly get enough channel access opportunities, resulting in poor end-to-end performance. Therefore, we propose an adaptive channel reservation MAC protocol based on forwarding traffic of key nodes, which is aimed at alleviating the congestion for key nodes. Nodes initiate reservations for future transmission time according to the buffer status before sending packets and then calculate the Weight of Reservation Ability (WRA). The node adaptively adjusts its reservation opportunity by comparing the WRA with neighbor nodes, thus improving the channel access efficiency and ensuring the transmission opportunity of key nodes. Extensive simulation confirms that our proposed FTKN-CRM provides significant improvements in end-to-end performance over the IEEE 802.11ax protocol and other reservation access protocols.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


